Small-mass effects in heavy-to-light form factors

We present the heavy-to-light form factors with two different non-vanishing masses at next-to-next-to-leading order and study its expansion in the small mass. The leading term of this small-mass expansion leads to a factorized expression for the form factor. The presence of a second mass results in a new feature, in that the soft contribution develops a factorization anomaly. This cancels with the corresponding anomaly in the collinear contribution. With the generalized factorization presented here, it is possible to obtain the leading small-mass terms for processes with large masses, such as muon-electron scattering, from the corresponding massless amplitude and the soft contribution.

==> figures/master6Top.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)},rotate=90]
		\path [draw=black,zigzag it,line width=0.25mm] (0,.62) -- (0,0);
		\draw [line width=0.6mm] (-1,-1.732)--(0,0);
		\draw [line width=0.6mm, dashed] (1,-1.732)--(0,0);
		\draw [snake it, line width=0.25mm] (0.85,-1.472)--(-0.425,-0.736);
		\draw [snake it, line width=0.25mm] (-0.85,-1.472)--(0.425,-0.736);
\end{tikzpicture}

==> figures/masterOffSunset0Mz.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\path [draw=black,zigzag it,line width=0.25mm] (-1.5,0) -- (-0.7,0);
		\path [draw=black,zigzag it,line width=0.25mm] (0.7,0) -- (1.5,0);
		\draw [line width=0.6mm] (-0.7,0)--(0.7,0);
		\centerarc [snake it, line width=0.25mm](0,0)(0:180:0.7)
		\centerarc [line width=0.6mm,dashed]((0,0)(180:360:0.7)
\end{tikzpicture}

==> figures/masterOffSunsetMMz.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\draw [line width=0.6mm,dashed] (-1.5,0) -- (1.5,0);
		\centerarc [line width=0.6mm](0,0)(0:180:0.7)
		\centerarc [line width=0.6mm]((0,0)(180:360:0.7)
\end{tikzpicture}

==> figures/masterOffSunsetMMzP1.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\draw [line width=0.6mm,dashed] (-1.5,0) -- (1.5,0);
		\centerarc [line width=0.6mm](0,0)(0:180:0.7)
		\centerarc [line width=0.6mm]((0,0)(180:360:0.7)
		\draw[fill=black,draw=none] (0,0.7) circle (3.5pt);
\end{tikzpicture}

==> figures/masterSunsetM00.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\draw [line width=0.6mm] (-1.5,0) -- (1.5,0);
		\centerarc [snake it, line width=0.25mm](0,0)(0:180:0.7)
		\centerarc [snake it, line width=0.25mm](0,0)(180:360:0.7)
\end{tikzpicture}

==> figures/masterSunsetMMM.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\draw [line width=0.6mm] (-1.5,0) -- (1.5,0);
		\centerarc [line width=0.6mm](0,0)(0:180:0.7)
		\centerarc [line width=0.6mm](0,0)(180:360:0.7)
\end{tikzpicture}

==> figures/masterSunsetMzz.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\draw [line width=0.6mm] (-1.5,0) -- (1.5,0);
		\centerarc [line width=0.6mm,dashed](0,0)(0:180:0.7)
		\centerarc [line width=0.6mm,dashed]((0,0)(180:360:0.7)
\end{tikzpicture}

==> figures/masterSunsetMzzP1.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\draw [line width=0.6mm] (-1.5,0) -- (1.5,0);
		\centerarc [line width=0.6mm,dashed](0,0)(0:180:0.7)
		\centerarc [line width=0.6mm,dashed]((0,0)(180:360:0.7)
		\draw[fill=black,draw=none] (0,0) circle (3.5pt);
\end{tikzpicture}

==> figures/masterSunsetz00.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\draw [line width=0.6mm,dashed] (-1.5,0) -- (1.5,0);
		\centerarc [snake it, line width=0.25mm](0,0)(0:180:0.7)
		\centerarc [snake it, line width=0.25mm]((0,0)(180:360:0.7)
\end{tikzpicture}

==> figures/masterSunsetzzz.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\draw [line width=0.6mm,dashed] (-1.5,0) -- (1.5,0);
		\centerarc [line width=0.6mm,dashed](0,0)(0:180:0.7)
		\centerarc [line width=0.6mm,dashed]((0,0)(180:360:0.7)
\end{tikzpicture}

==> figures/masterTadpoleMM.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\centerarc [line width=0.6mm](-0.6,0)(0:360:0.6)
		\centerarc [line width=0.6mm](0.6,0)(0:360:0.6)
\end{tikzpicture}


==> figures/masterTadpolezM.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\centerarc [line width=0.6mm](-0.6,0)(0:360:0.6)
		\centerarc [line width=0.6mm,dashed](0.6,0)(0:360:0.6)
\end{tikzpicture}


==> figures/masterTadpolezz.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)}]
		\centerarc [line width=0.6mm,dashed](-0.6,0)(0:360:0.6)
		\centerarc [line width=0.6mm,dashed](0.6,0)(0:360:0.6)
\end{tikzpicture}


==> figures/masterTriBub12MMMz.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)},rotate=90]
		\path [draw=black,zigzag it,line width=0.25mm] (0,.62) -- (0,0);
		\draw [line width=0.6mm] (-1,-1.732)--(0,0);
		\draw [line width=0.6mm, dashed] (1,-1.732)--(0,0);
		\centerarc [line width=0.6mm](0,0)(240:300:1.7)
		\centerarc [line width=0.6mm](0,-2.944)(60:120:1.7)
\end{tikzpicture}

==> figures/masterTriBub12Mz00.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)},rotate=90]
		\path [draw=black,zigzag it,line width=0.25mm] (0,.62) -- (0,0);
		\draw [line width=0.6mm] (-1,-1.732)--(0,0);
		\draw [line width=0.6mm,dashed] (1,-1.732)--(0,0);
		\centerarc [snake it, line width=0.25mm](0,0)(240:300:1.7)
		\centerarc [snake it, line width=0.25mm](0,-2.944)(60:120:1.7)
\end{tikzpicture}

==> figures/masterTriBub12Mzzz.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)},rotate=90]
		\path [draw=black,zigzag it,line width=0.25mm] (0,.62) -- (0,0);
		\draw [line width=0.6mm] (-1,-1.732)--(0,0);
		\draw [line width=0.6mm,dashed] (1,-1.732)--(0,0);
		\centerarc [line width=0.6mm,dashed](0,0)(240:300:1.7)
		\centerarc [line width=0.6mm,dashed](0,-2.944)(60:120:1.7)
\end{tikzpicture}

==> figures/masterTriTriMMz0.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)},rotate=90]
		\path [draw=black,zigzag it,line width=0.25mm] (0,.62) -- (0,0);
		\draw [line width=0.6mm] (-1,-1.732)--(0,0);
		\draw [line width=0.6mm, dashed] (1,-1.732)--(0,0);
		\draw [snake it, line width=0.25mm] (-0.85,-1.472)--(0.85,-1.472);
		\draw [snake it, line width=0.25mm] (0.85,-1.472)--(-0.425,-0.736);
\end{tikzpicture}

==> figures/masterTriTriMzz0.tex <==
\begin{tikzpicture}[scale=.9,baseline={(0,0)},rotate=90]
		\path [draw=black,zigzag it,line width=0.25mm] (0,.62) -- (0,0);
		\draw [line width=0.6mm] (-1,-1.732)--(0,0);
		\draw [line width=0.6mm, dashed] (1,-1.732)--(0,0);
		\draw [snake it, line width=0.25mm] (-0.85,-1.472)--(0.85,-1.472);
		\draw [snake it, line width=0.25mm] (-0.85,-1.472)--(0.425,-0.736);
\end{tikzpicture}
